Towards Generic Image Manipulation Detection with Weakly-Supervised Self-Consistency Learning

As advanced image manipulation techniques emerge, detecting the manipulation becomes increasingly important. Despite the success of recent learning-based approaches for image manipulation detection, they typically require expensive pixel-level annotations to train, while exhibiting degraded performance when testing on images that are differently manipulated compared with training images. To address these limitations, we propose weakly-supervised image manipulation detection, such that only binary image-level labels (authentic or tampered with) are required for training purpose. Such a weakly-supervised setting can leverage more training images and has the potential to adapt quickly to new manipulation techniques. To improve the generalization ability, we propose weakly-supervised self-consistency learning (WSCL) to leverage the weakly annotated images. Specifically, two consistency properties are learned: multi-source consistency (MSC) and inter-patch consistency (IPC). MSC exploits different content-agnostic information and enables cross-source learning via an online pseudo label generation and refinement process. IPC performs global pair-wise patch-patch relationship reasoning to discover a complete region of manipulation. Extensive experiments validate that our WSCL, even though is weakly supervised, exhibits competitive performance compared with fully-supervised counterpart under both in-distribution and out-of-distribution evaluations, as well as reasonable manipulation localization ability.

==> figures/fig-impression.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/impression.pdf}
    \caption{Manipulation detection result comparison between unsupervised
    method (CFA1~\cite{ferrara2012image}), fully-supervised method
    (Mantra-Net~\cite{wu2019mantra} and MVSS-Net~\cite{chen2021image}), and our
    weakly-supervised method.}
    \label{fig:impression}
\end{figure}


==> tables/tab-comparison-with-sota-combined.tex <==
\begin{table}
    \centering
    \caption{Comparison with state-of-the-art unsupervised and fully-supervised
    methods on the combined F1 score under decision threshold $0.5$.}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|cccc}
            \hline
            Sup. & Method & Columbia & CASIAv1 & Coverage & IMD2020 \\
            \hline
            \hline
            \multirow{2}{*}{Unsup.} & NOI1~\cite{mahdian2009using} & 0.000 &
            0.000 & 0.000 & 0.000 \\
            & CFA1~\cite{ferrara2012image} & 0.000 & 0.000 & 0.000 & 0.000 \\
            \hline
            \multirow{5}{*}{Pixel} & ManTra-Net~\cite{wu2019mantra} & 0.000 & 
            0.000 & 0.000 & 0.000 \\
            & CR-CNN~\cite{yang2020constrained} & 0.413 & 0.382 & 0.181 & - \\
            & GSR-Net~\cite{zhou2020generate} & 0.042 & 0.042 & 0.000 & - \\
            & FCN~\cite{chen2021image} & 0.305 & 0.562 & 0.189 & 0.217 \\
            & MVSS-Net~\cite{chen2021image} & \textbf{0.711} & \textbf{0.565} &
            \textbf{0.317} & \textbf{0.375} \\
            \hline
            \multirow{2}{*}{Image} & FC-MIL~\cite{pathak2014fully} & 0.041 &
            0.053 & 0.109 & 0.211 \\
            & Ours & 0.235 & 0.311 & 0.219 & 0.250 \\
            & Ours (tricks) & 0.331 & 0.232 & 0.171 & 0.263 \\
            & Ours (superpixel) & 0.364 & 0.265 & 0.260 & 0.269 \\
            \hline
        \end{tabular}
    }
    \label{tab:comp-with-sota-combined}
\end{table}

==> tables/tab-novel-dataset-and-ablation-pool.tex <==
\begin{table*}
    \begin{minipage}[h]{0.6\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{c|cccc|cccc|c|c}
            \hline 
            \multirow{2}{*}{Method} & \multicolumn{4}{c|}{GIER} & \multicolumn{4}{c|}{IEdit} & \multicolumn{2}{c}{\cellcolor{mygray}Avg}\tabularnewline
             & AUC $\uparrow$ & Spe. $\uparrow$ & Sen. $\uparrow$ & I-F1 $\uparrow$ & AUC $\uparrow$ & Spe. $\uparrow$ & Sen. $\uparrow$ & I-F1 $\uparrow$ & \cellcolor{mygray}AUC $\uparrow$ & \cellcolor{mygray}I-F1 $\uparrow$\tabularnewline
            \hline 
            \hline 
            FCN+DA~\cite{chen2021image} & 0.507 & 0.310 & 0.692 & \underline{0.428} & 0.539 & 0.389 & 0.658 & 0.489 & \cellcolor{mygray}0.523 & \cellcolor{mygray}\underline{0.458}\tabularnewline
            \hline 
            MVSS-Net~\cite{chen2021image} & 0.510 & 0.204 & 0.804 & 0.325 & 0.537 & 0.598 & 0.463 & 0.522 & \cellcolor{mygray}0.524 & \cellcolor{mygray}0.424\tabularnewline
            \hline 
            Ours & \underline{0.577} & 0.192 & 0.869 & 0.315 & \underline{0.551} & 0.536 & 0.537 & \underline{0.537} & \cellcolor{mygray}\underline{0.564} & \cellcolor{mygray}0.426\tabularnewline
            \hline 
            Ours + fine-tune & \textbf{0.593} & 0.431 & 0.657 & \textbf{0.521} & \textbf{0.589} & 0.593 & 0.566 & \textbf{0.577} & \cellcolor{mygray}\textbf{0.591} & \cellcolor{mygray}\textbf{0.549}\tabularnewline
            \hline 
        \end{tabular}%
        }
        \caption{Comparison with state-of-the-art fully-supervised methods on
        novel datasets in terms of image-level detection.}
        \label{tab:novel-datasets}
    \end{minipage}
    \hfil
    \begin{minipage}[h]{0.38\linewidth}
        \centering
        \resizebox{0.8\linewidth}{!}{%
            \begin{tabular}{>{\centering}p{1.7cm}|>{\centering}p{0.9cm}>{\centering}p{0.9cm}>{\centering}p{0.9cm}>{\centering}p{0.9cm}}
            \hline 
            Method & AUC & I-F1 & P-F1 & C-F1\tabularnewline
            \hline 
            \hline 
            Max Pool & 0.569 & 0.551 & 0.088 & 0.152\tabularnewline
            \hline 
            Avg Pool & 0.563 & 0.312 & 0.069 & 0.113\tabularnewline
            \hline 
            GeM~\cite{radenovic2018fine} & 0.618 & \underline{0.342} & 0.103 & 0.158\tabularnewline
            \hline 
            GSM~\cite{wang2017learning} & \underline{0.638} & \textbf{0.372} & \underline{0.107} & \underline{0.166}\tabularnewline
            \hline 
            Otsu & \textbf{0.641} & 0.340 & \textbf{0.120} & \textbf{0.177}\tabularnewline
            \hline 
            \end{tabular}%
        }
        \caption{Comparison on different pooling methods for multiple instance
        learning.}
        \label{tab:pooling}
    \end{minipage}
\end{table*}
